Neuron detection in stack images: a persistent homology interpretation

Automation and reliability are the two main requirements when computers are applied in Life Sciences. In this paper we report on an application to neuron recognition, an important step in our long-term project of providing software systems to the study of neural morphology and functionality from biomedical images. Our algorithms have been implemented in an ImageJ plugin called NeuronPersistentJ, which has been validated experimentally. The soundness and reliability of our approach are based on the interpretation of our processing methods with respect to persistent homology, a well-known tool in computational mathematics.

==> algorithmic1.tex <==
\section{Algorithmic background and method}\label{sec:abam}


\subsection{The method}

\begin{figure}
\centering

\subfigure{%
            \label{maximum}
            \includegraphics[scale=0.1]{mp1.png}
        }%
        \subfigure{%
           \label{maximum_filter}
           \includegraphics[scale=0.1]{mp0.png}
        }
        \subfigure{%
            \label{maximum_filter_hold}
            \includegraphics[scale=0.1]{mp2.png}
        }
\caption{From left to right. (a) Maximum intensity projection from a z-stack. (b) Maximum intensity projection
with a median filter. (c) Huang's thresholding method applied to the image of Figure~\ref{maximum_filter}.}
\end{figure}

Our method to detect the neuronal structure from images, like the one of Figure~\ref{maximum}, can be split into two steps,
which will be called respectively \emph{salt-and-pepper removal} and \emph{persistent}. In the former one, we reduce the
salt-and-pepper noise, and in the latter one we dismiss the elements which appear in the image but which are not part of the
structure of the main neuron (astrocytes, other neurons and so on). 

In order to carry out the task of reducing the salt-and-pepper noise, we apply the following process both to the images
of the stack and to the maximum intensity projection image. Firstly, we apply a \emph{low-pass filter}~\cite{Cas96} to the images.
In our case, the filter which fits better with our problem is the \emph{median} one, since such a filter reduces speckle noise
while retaining sharp edges. The filter length is set to $10$ pixels for the situation described in Section~\ref{sec:bpaia}, 
this value has been pragmatically determined and it is the only parameter of the whole method which must be changed if
the acquisition procedure is modified. The result produced for the maximum intensity projection image of 
Figure~\ref{maximum} is shown in Figure~\ref{maximum_filter}.

Afterwards, we obtain binary images using \emph{Huang's method}~\cite{Huang}. This procedure automatically determines an adequate threshold 
value for the images. Applying that method to the image of Figure~\ref{maximum_filter}, we obtain the result depicted in 
Figure~\ref{maximum_filter_hold}.

However, in the image of Figure~\ref{maximum_filter_hold} we can see elements which does not belong
to the main neuronal structure. Let us explain how we manage to remove those undesirable elements. 

It is worth noting that in every slide of a z-stack appears part of the neuronal structure. On the contrary, 
irrelevant elements just appear in some of the slides. This will be the key idea of our method. 

More concretely, we proceed as follows. As we have explained previously, we apply the \emph{salt-and-pepper removal}
step to all the slides of the z-stack, the result of that in our case study can be seen in Figure~\ref{processed_stack}. 
 
\begin{figure}
\centering
\begin{tikzpicture}
\draw (0,0) node {\includegraphics[scale=0.075]{stack/2_8_hold.png}}; 
\draw (3,0) node {\includegraphics[scale=0.075]{stack/3_8_hold.png}}; 
\draw (6,0) node {\includegraphics[scale=0.075]{stack/4_8_hold.png}};
\draw (9,0) node {\includegraphics[scale=0.075]{stack/1_8_hold.png}};  
\draw (0,-3) node {\includegraphics[scale=0.075]{stack/5_8_hold.png}};  
\draw (3,-3) node {\includegraphics[scale=0.075]{stack/6_8_hold.png}}; 
\draw (6,-3) node {\includegraphics[scale=0.075]{stack/7_8_hold.png}}; 
\draw (9,-3) node {\includegraphics[scale=0.075]{stack/8_8_hold.png}}; 
\end{tikzpicture}
\caption{Processed z-stack of a neuron}\label{processed_stack}
\end{figure}

In the \emph{persistent} step, we firstly construct a \emph{filtration} of the binary image associated with the maximum projection image. A
monochromatic image, ${\mathcal D}$, can be seen as a set of black pixels (which represent the foreground of the image), and
a \emph{filtration} of ${\mathcal D}$ is a nested subsequence of images $D^0 \subseteq D^1 \subseteq \ldots \subseteq D^m = \mathcal{D}$.
 
In order to construct a filtration of the binary image associated with the maximum projection image we proceed as follows. 
$D^m$ is the maximum projection image. $D^{m-1}$ consists of the connected components of $D^m$ 
whose intersection with the first slide of the stack is non empty. $D^{m-2}$ consists of the connected components of $D^{m-1}$ 
whose intersection with the second slide of the stack is non empty, and so on. In general,  $D^{m-n}$ consists of the connected components of $D^{m-n+1}$
whose intersection with the $n$-th slide of the stack is non empty. In this way, a filtration of the maximum projection image is obtained, see 
Figure~\ref{filtration_processed_stack}. 

  \begin{figure}
  \centering
  \begin{tikzpicture}
  \draw (0,0) node {\includegraphics[scale=0.075]{stack/5_8_hold_filt.png}}; 
  \draw (1.5,0) node {$\subseteq$};
  \draw (0,-1.25) node {$D^0$};
  \draw (3,0) node {\includegraphics[scale=0.075]{stack/5_8_hold_filt.png}}; 
  \draw (4.5,0) node {$\subseteq$};
  \draw (3,-1.25) node {$D^1$};
  \draw (6,0) node {\includegraphics[scale=0.075]{stack/5_8_hold_filt.png}};
  \draw (7.5,0) node {$\subseteq$};
  \draw (6,-1.25) node {$D^2$};
  \draw (9,0) node {\includegraphics[scale=0.075]{stack/5_8_hold_filt.png}};  
  \draw (10.5,0) node {$\subseteq$};
  \draw (9,-1.25) node {$D^3$};
  \draw (0,-3) node {\includegraphics[scale=0.075]{stack/5_8_hold_filt.png}};  
  \draw (1.5,-3) node {$\subseteq$};
  \draw (0,-4.25) node {$D^4$};
  \draw (3,-3) node {\includegraphics[scale=0.075]{stack/6_8_hold_filt.png}}; 
  \draw (4.5,-3) node {$\subseteq$};
  \draw (3,-4.25) node {$D^5$};
  \draw (6,-3) node {\includegraphics[scale=0.075]{stack/7_8_hold_filt.png}}; 
  \draw (7.5,-3) node {$\subseteq$};
  \draw (6,-4.25) node {$D^6$};
  \draw (9,-3) node {\includegraphics[scale=0.075]{stack/8_8_hold_filt.png}};
  \draw (10.5,-3) node {$\subseteq$};
  \draw (9,-4.25) node {$D^7$};
  \draw (4.5,-6) node {\includegraphics[scale=0.06]{stack/maximum_projection_filter_hold.png}}; 
  \draw (4.5,-7.25) node {$D^8$};
  \end{tikzpicture}
  \caption{Filtration of the maximum projection image}\label{filtration_processed_stack}
  \end{figure}

As we know that the neuron appears in all the slides of the stack, the component $D^0$ of our filtration
will be the structure of the neuron. As a final remark, we can notice that the construction of the 
filtration reaches a point where it is stable; that is, a level of the filtration $D^i$ of the filtration 
such that $D^j$ is equal to $D^i$ for all $0\leq j < i$. An example can be seen in the components 
$D^0$ to $D^4$ of Figure~\ref{filtration_processed_stack}. This observation will be important in the next
subsection. 
 

\subsection{Interpretation in terms of persistent homology}

The persistent adjective of the second step of the method presented in the previous subsection comes from
the nice interpretation which can be given in terms of the \emph{persistent homology theory}~\cite{ELZ02},
a branch of Algebraic Topology~\cite{Mau96}. In a nutshell, persistent homology is a technique which 
allows one to study the \emph{lifetimes} of \emph{topological attributes}. A detailed description of persistent homology can
be seen in~\cite{ELZ02,PHDZomorodian}, here we just present the main ideas.

One of the most important notions in Algebraic Topology is the one of \emph{homology groups}. The homology group in dimension
$n$ of an object $X$, denoted by $H_n(X)$, is a set which consists of the $n$ dimensional holes of $X$, also called \emph{$n$ dimensional
homology classes} of $X$. To be more concrete, $H_0(X)$ measures the number of connected components of $X$, and the
homology groups $H_n(X)$, with $n>0$, measure higher dimensional connectedness. In the case of $2$ dimensional monochromatic images, 
the $0$ and $1$ dimensional homology classes are, respectively, the connected components and the holes of the image; there are not homology classes 
in higher dimensions. 

Now, given a $2$ dimensional monochromatic digital image ${\mathcal{D}}$ and a filtration 
$D^0 \subseteq D^1 \subseteq \ldots \subseteq D^m = \mathcal{D}$ of ${\mathcal{D}}$, a $n$-homology class $\alpha$ \emph{is born} at $D^i$ if it belongs to the set $H_n(D^i)$ 
but not to $H_n(D^{i-1})$. 
Furthermore, if $\alpha$ is born at $D^i$ it \emph{dies entering} $D^j$, with $i<j$, if it belongs to the set $H_n(D^{j-1})$ but not to
$H_n(D^{j})$. The \emph{persistence} of $\alpha$ is $j-i$. We may represent the lifetime of a homology class as an interval, and we
define a \emph{barcode} to be the set of resulting intervals of a filtration. 

In the case of the filtrations presented in the previous subsection, the outstanding barcode is the one of $0$ dimensional homology classes.
It is worth noting that the structure of the neuron lives from the beginning to the end of the filtration while 
external elements are short-lived. 

For example, the barcode associated with the filtration of Figure~\ref{filtration_processed_stack} is the one depicted in Figure~\ref{barcode}. 

\begin{figure}
\centering
\includegraphics[scale=.5]{barcode.png}
\caption{Barcode of the filtration of Figure~\ref{filtration_processed_stack}}\label{barcode}
\end{figure}

Let us analyze the information which can be extracted from such barcode. There are several connected components which live is reduced to the 
maximum projection image, the green connected components of Figure~\ref{maximum_filter_hold_color}, and can be considered as noise.
Notwithstanding that the components $x_1,x_2$ and $x_3$ (which are respectively the red, yellow and orange connected components of 
Figure~\ref{maximum_filter_hold_color}) live a bit longer than green components; they are also short-lived; so, they cannot be part of the main structure
of the neuron, it is likely that these components come from other biological elements. Eventually, we have the $x_0$ component, the blue
connected component of Figure~\ref{maximum_filter_hold_color}, which lives from the beginning to the end of the filtration; therefore, as it lives from the
beginning to the end of the filtration, it represents the structure of the neuron. 

\begin{figure}
\centering
\includegraphics[scale=0.2]{TracingColor.png}
\caption{Connected components of the projection}\label{maximum_filter_hold_color}
\end{figure}

We have devised an efficient algorithm to obtain the barcode of $0$ dimensional homology classes associated with
the images that we have presented in the previous subsection. This method takes advantage of both the way of building
the filtration and the stability of such a filtration. Firstly, we obtain the connected components of the level $0$
of the filtration, $D^0$; this is a well-known process called \emph{connected component labeling} which can be solved
using different efficient algorithms, see~\cite{ccl10,Lee07}. Such connected components are $0$ dimensional homology
classes which are born at $D^0$ and live until the end of the filtration, this fact comes from the filtration 
construction process. Now, we focus on the level $1$ of the filtration, $D^1$. As we have seen at the end of the
previous subsection, the filtration has a stability level; therefore, we consider two feasible cases. 
If $D^0$ is equal to $D^1$, we can pass to the next level of the filtration. Otherwise, we obtain the connected components
which appear at $D^1$ but not at $D^0$, such components are $0$ dimensional homology classes which are born at $D^1$
and live until the end of the filtration. In order to check if $D^0$ and $D^1$ are equal, we use the 
\emph{MD6 Message-Digest Algorithm}~\cite{MD6}. Such algorithm is a cryptographic hash function which given an image
returns a \emph{unique} string; therefore, if the result produced for $D^0$ and $D^1$ is the same, we can claim that both
images are equal. This procedure is faster than comparing pixel by pixel the images.

The above process is iterated for the rest of the levels of the filtration. In general, if we are in the level $i$ of
the filtration, there are two cases: if $D^{i-1} = D^i$ (this is tested with MD6 algorithm) then pass to level $i+1$; otherwise
the connected components which appear in $D^i$ but not in $D^{i-1}$ are the $0$ dimensional homology classes which are born at $D^i$
and live until the end of the filtration. In this way, we can obtain the barcode of $0$ dimensional homology classes without
explicitly computing persistent homology.




==> experimental__Copia_conflictiva_de_J__nathan_Heras_2012-07-04_.tex <==
\section{Experimental results}\label{sec:er}

The procedure to detect neural structure presented in the previous section has been implemented
as a new plugin for \emph{ImageJ}~\cite{ImageJ} called \emph{NeuronPersistentJ}~\cite{NeuronPersistentJ}. 

We have validated our method and plugin with a set of image stacks of real 3D neuron dendrites acquire
using the procedure explained in Section~\ref{sec:bpaia}. In order to test the suitability of our software,
we have compared a manual tracing with the results obtained using NeuronPersistentJ. In particular, we
have considered the following relevant features: number of branches, area of the region of interest, 


The experimental results that we have obtained with our dataset are shown in Table~\ref{table}.  


\begin{table}
{%
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & Number of & Area of  & Percentage of \\
& branches & region of interest & neuron \\
\hline
Effectiveness  & 100$\%$ &  &  \\
of the method & & &\\
\hline
\end{tabular}
\end{center}
}%
\caption{Computational times}\label{table}
\end{table}


Figure~\ref{Examples} illustrates the results which are obtained with our plugin with three different examples. 


\begin{figure}
\centering

\subfigure{%
            \label{maximum}
            \includegraphics[scale=0.1]{stack1.png}
        }%
        \subfigure{%
           \label{maximum_filter}
           \includegraphics[scale=0.1]{stack2.png}
        }
        \subfigure{%
            \label{maximum_filter_hold}
            \includegraphics[scale=0.1]{stack3.png}
        }\\
\subfigure{%
            \label{maximum}
            \includegraphics[scale=0.1]{Tracing1.png}
        }%
        \subfigure{%
           \label{maximum_filter}
           \includegraphics[scale=0.1]{Tracing2.png}
        }
        \subfigure{%
            \label{maximum_filter_hold}
            \includegraphics[scale=0.1]{Tracing3.png}
        }
\caption{In the top the maximum projection of three stacks. In the bottom the tracings obtained with NeuronPersistentJ}\label{Examples}
\end{figure}


